DAIS: Dependency-Aware Intermediate QA Supervision for Complex Reasoning

Chain-of-thought (CoT) supervision exposes intermediate rationales, but flat rationale targets usually optimize a single reasoning sequence and provide limited supervision on how local conclusions should support later decisions. We introduce Dependency-Aware Intermediate QA Supervision (DAIS), a training-time framework that converts filtered teacher rationales into stage-level QA records. Each intermediate record predicts a local answer conditioned on the previous states needed for that decision, while the final-answer record keeps the original task format; evaluation therefore uses only the original input and optional context. Across GDPR, AIACT, MedQA, and FOLIO with multiple Qwen backbones, DAIS improves average final-answer accuracy over answer-only, flat chain-of-thought, and independent-QA baselines. On policy-compliance benchmarks, it achieves a largest gain of 5.6% and an average gain of 4.2% over the strongest non-DAIS baseline. Controlled ablations show that valid previous-state conditioning contributes beyond longer targets or additional intermediate text, supporting dependency-conditioned intermediate QA as a lightweight auxiliary supervision signal for standard final-answer inference.

==> prompts.tex <==
folio：

You are a strict evaluation assistant.

Your task is to evaluate whether the predicted label matches the gold label.

Step 1: Extract the final label from the prediction.
Step 2: Normalize labels using the following mapping:

- True
- False
- Unknown

Step 3: Compare the normalized prediction with the gold label.

Prediction:
{prediction}

Gold Label:
{i['output']}

Output:
- 1 if correct
- 0 if incorrect

Output only 0 or 1."""





medqa:


You are an expert evaluator for medical multiple-choice question answering.

Your task is to determine whether the model's final answer is correct.

You will be given:
1. A medical question
2. Multiple-choice options
3. The ground-truth answer
4. A model-generated response

You must carefully identify the FINAL answer selected by the model.

Evaluation Rules:
- Focus ONLY on the model's final selected answer.
- Ignore intermediate reasoning if the final conclusion is different.
- The answer may appear as:
  - option letter (e.g. "A")
  - option content
  - both
  - natural language equivalent
- If the model expresses uncertainty but finally selects the correct answer, mark correct.
- If multiple conflicting answers appear, use the LAST explicit final answer.
- If no clear final answer exists, mark incorrect.
- Be strict.
- Do not use outside medical knowledge beyond the provided ground truth.

Question:
{i['question']}

Options:
A. {i['options'].get('A', '')}
B. {i['options'].get('B', '')}
C. {i['options'].get('C', '')}
D. {i['options'].get('D', '')}
E. {i['options'].get('E', '')}

Ground Truth:
Option: {i['answer_idx']}
Content: {i['answer']}

Model Response:
{prediction}

Return ONLY valid JSON:

{{
    "predicted_answer": "extracted final answer",
    "is_correct": true,
    "confidence": "high/medium/low"
}}





gdpr and aiact:
You are a strict evaluation assistant.

Your task is to evaluate whether the predicted label matches the gold label.

Step 1: Extract the final label from the prediction.
Step 2: Normalize labels using the following mapping:

- permit or permitted → permit
- prohibit or prohibited → prohibit
- unrelate or unrelated or not applicable→ not applicable

Step 3: Compare the normalized prediction with the gold label.

Prediction:
{prediction}

Gold Label:
{i['output']}

Output:
- 1 if correct
- 0 if incorrect

Output only 0 or 1.

==> schema_example.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{p{0.28\linewidth}p{0.62\linewidth}}
\toprule
\textbf{Task domain} & \textbf{Example induced subtask schema} \\
\midrule
Legal / policy compliance
&
Legal element extraction;
applicable rule matching;
condition or exception checking;
compliance inference. \\

Medical QA
&
Clinical concept mapping;
clinical evidence grounding;
differential comparison;
mechanistic causal inference;
clinical decision making. \\
\bottomrule
\end{tabular}
\caption{
Examples of dataset-level subtask schemas.
The induced schema normalizes recurring subtask candidates within a dataset.
Final-answer prediction is handled separately by the final QA state.
}
\label{tab:schema_examples}
\end{table}
